K-Diag: Knowledge-enhanced Disease Diagnosis in Radiographic Imaging

In this paper, we consider the problem of disease diagnosis. Unlike the conventional learning paradigm that treats labels independently, we propose a knowledge-enhanced framework, that enables training visual representation with the guidance of medical domain knowledge. In particular, we make the following contributions: First, to explicitly incorporate experts' knowledge, we propose to learn a neural representation for the medical knowledge graph via contrastive learning, implicitly establishing relations between different medical concepts. Second, while training the visual encoder, we keep the parameters of the knowledge encoder frozen and propose to learn a set of prompt vectors for efficient adaptation. Third, we adopt a Transformer-based disease-query module for cross-model fusion, which naturally enables explainable diagnosis results via cross attention. To validate the effectiveness of our proposed framework, we conduct thorough experiments on three x-ray imaging datasets across different anatomy structures, showing our model is able to exploit the implicit relations between diseases/findings, thus is beneficial to the commonly encountered problem in the medical domain, namely, long-tailed and zero-shot recognition, which conventional methods either struggle or completely fail to realize.

==> miccai2023 (1)/contents/conclusion.tex <==
\section{Conclusion}
\vspace{-.2cm}
In this paper, we propose a novel knowledge-enhanced classification model,  that enables learning visual representation by exploiting the relationship between different medical concepts in the knowledge graph.
While conducting thorough experiments on x-ray image datasets across different anatomy structures, we show that injecting medical prior knowledge is beneficial for tackling (i) long-tailed recognition, (ii) zero-shot recognition.
As for future work, we plan to generalize the idea towards self-supervised learning on pairs of image and text reports and more diverse modalities.

%Moreover, we analyse on the assembling dataset CXR-Mix, proving the superiority of our model on effectively exploiting knowledge across datasets and annotation classes.
%Finally, we show the visualization of our grounding results making our predication more credible.

%First, we propose a knowledge encoder to build a neural representation of a knowledge base in the textural embedding space.
%Second, we propose a learnable prompt module to implicit decompose the medical concepts and regularize the embedding space.
%Third, we adopt a transformer-based disease-query module for cross-modality fusion, providing interoperability for prediction.
%We conduct thorough experiments to validate the effectiveness of our proposed architecture on three disease diagnosis datasets across different anatomy structures.
%Moreover, we analyse on the assembling dataset CXR-Mix, proving the superiority of our model on effectively exploiting knowledge across datasets and annotation classes.
%Finally, we show the visualization of our grounding results making our predication more credible.
%\weidi{give an initial version, I'll edit it afterwards}\chaoyi{fixed}


==> miccai2023 (1)/contents/experiment.tex <==
\section{Experiments}


\subsection{Datasets}
In this paper, we conduct experiments on datasets of X-ray images, 
due to there exists sufficient data across anatomy structures and annotated pathology categories in this field, supporting thorough evaluation.

%\weidi{need a summary sentence, ``In this paper, we consider ..... why ? because abundant data ? or some reason.'' }

\vspace{5pt} \noindent \textbf{VinDr-PCXR~\cite{Nguyen2022VinDrPCXRAO}}
is a new pediatric CXR dataset of 9,125 studies, which was officially divided into a training set and a test set of 7,728 and 1,397 studies respectively. Each scan in the training set was manually annotated for the presence of 15 diseases by a pediatric radiologist who has more than ten years of experience,
while in the official test set, there are 11 diseases.
Additionally, for fair and robust evaluation, 
we further merged the rare diseases~(positive samples less than 5) into ``other diseases'',
resulting in only 6 classes in the test set, including no finding, bronchitis, broncho-pneumonia, other disease, bronchiolitis, and pneumonia.

%\textcolor{blue}{For , 
%we merged them into "other diseases", resulting in 6 classes, }
%\weidi{I don't understand the last sentence, 
%why it's 6 classes, how does the number change from 15 to 6?}

\vspace{5pt} \noindent \textbf{VinDr-Mammo~\cite{Nguyen2022VinDrMammoAL}}
is a full-field digital mammography dataset comprising 20,000 images~(5,000 four-view scans). Each scan was manually annotated for no finding or the presence of 10 mammography findings, including mass, calcification, asymmetry, focal asymmetry, global asymmetry, architectural distortion, and suspicious lymph node, skin thickening, skin retraction, nipple retraction. The dataset was official divided into a training set and a test set with 4,000 and 1,000 exams respectively.

\vspace{5pt} \noindent \textbf{VinDr-SpineXr~\cite{Nguyen2021VinDrSpineXRAD}}
is a spine X-ray dataset comprising 10,468 spine X-ray images from 5,000 studies. 
Each image was manually annotated by an experienced radiologist with no finding or abnormal findings in 7 categories, including osteophytes, foraminal stenosis, vertebral collapse, disc space narrowing, spondylolysthesis, surgical implant, and other lesions. 
The dataset was official divided into a training set a test set of 4,000 and 1,000 studies respectively.

\vspace{5pt} \noindent \textbf{PadChest~\cite{bustos2020padchest}} is a chest X-ray dataset with 160,868 chest X-ray images labeled with 174 different radiographic findings, 19 differential diagnoses, only $27\%$ of the labels~(totaling 39,053 examples) come from board-certified radiologists, and the rest are obtained by using a recurrent neural network with attention trained on the radiology reports. 
For evaluation purposes, we only test on samples annotated by board-certified radiologists, and report the zero-shot test results.

\vspace{5pt} \noindent \textbf{CXR-Mix.}
In this paper, we also construct a dataset by assembling 11 public datasets, 
including {ChestXray-14~\cite{wang2017chestx}}
{GoogleNIH~\cite{majkowska2020chest}}
{Covid-CXR2~\cite{pavlova2021covid}}
{CheXpert~\cite{irvin2019chexpert}}
{Object-CXR~\cite{objectcxr}}
{NLM-TB~\cite{jaeger2014two}}
{RSNA~\cite{shih2019augmenting}}
{SIIM-ACR~\cite{filice2020crowdsourcing}}
{VinDR~\cite{nguyen2022vindr}}
{OpenI~\cite{demner2016preparing}}
{MIMIC-CXR~\cite{johnson2019mimic}},
termed as \textbf{CXR-Mix}.
We refer the readers to~\cite{cohen2022torchxrayvision} for more details of these datasets. For the datasets~\cite{wang2017chestx,irvin2019chexpert} with official train/val/test splits, we use them directly, 
for those~\cite{majkowska2020chest,nguyen2022vindr,pavlova2021covid,objectcxr} with official train/test splits, 
we random split the train split with $0.8/0.2$ for train/val, in other cases, 
we randomly split the datasets~\cite{shih2019augmenting,filice2020crowdsourcing,jaeger2014two,demner2016preparing,johnson2019mimic} with $0.7/0.1/0.2$ for train/val/test. 
As a result, our constructed CXR-Mix ends up with $763,520$ chest X-rays for training, 
$28, 925$ for val, and $28,448$ for test, spanning across a total of $38$ classes in the CXR-Mix. 
\textbf{Note that}, each of these datasets was originally collected to serve different purposes, 
the annotations are often partially available,  
for example, the images from the  pneumonia dataset lack labels for pneumothorax, 
we use $-1$ to denote the label missing and will not calculate the final CE loss on them.

% on the 106 unseen radiographic findings with positive samples larger than 50 in the dataset.

\subsection{Implementation and Training Details}

\vspace{5pt} \noindent \textbf{Knowledge-Enhanced Text Encoder.}
To construct the knowledge encoder, we initialize the text encoder from ClinicalBERT~\cite{alsentzer2019publicly}, and finetune it for 100K training steps.
In each mini-batch, 64 concept-definition pairs are used for training.
We set the maximal sequence length as 256, though the definition could be long sometimes.
We use AdamW~\cite{loshchilov2017decoupled} as the optimizer with $lr =1\times 10^{-4}$ and $lr_\text{warm up} = 1\times 10^{-5}$. 

\vspace{5pt} \noindent \textbf{Knowledge-Enhanced Classification Framework.}
We freeze the knowledge encoder and set other parts to be learnable, 
{\em i.e.}, visual encoder, prompt module, disease-query module.
We train the model for 100 epochs with batch size 128, 
and use AdamW~\cite{loshchilov2017decoupled} is adopted as the optimizer with $lr =1\times 10^{-4}$ and $lr_\text{warm up} = 1\times 10^{-5}$. 


==> miccai2023 (1)/contents/introduction.tex <==
\section{Introduction}

The application of artificial intelligence (AI) has delivered impressive results in diagnosing diseases from medical scans~\cite{Mirbabaie2021}. 
A commonly adopted framework is to train vision models by supervised learning with discrete labels and predict pathology categories within a fixed-size vocabulary at inference time~\cite{cohen2022torchxrayvision,Zhou2022longtail}.
However, such a learning paradigm suffers from two limitations: 
{\em first}, the model is unable to generalize toward previously unseen categories;
{\em second}, the labels are converted into one-hot vectors as illustrated in Fig.~\ref{fig:intuition}, that are \textbf{orthogonal} in the embedding space, 
leaving the intrinsic relations between different pathologies or diseases unexploited.



In the recent literature, 
jointly training visual-language models has shown promising progress in computer vision~\cite{pratt2022does,radford2021learning}, often called Foundation Models. 
For example, CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling} have 
demonstrated remarkable ``zero-shot'' generalization for various downstream tasks by learning the joint representation of image and text with simple noise contrastive learning. Crucially, the data used to train these powerful foundation models can simply be crawled from the Internet without laborious manual annotation.
% actions, objects, human-object interactions, and object-object relationships. 
% As a result, these pre-trained foundation models have demonstrated remarkable ``zero-shot'' generalization for various image classification tasks. 
% Crucially, the data used to train these powerful foundation models can simply be crawled from the Internet at scale, without any laborious manual annotation.
% \weidi{you need to edit the above sections, as it is copied from my other paper, rewrite or short it. }
However, as commonly known, 
collecting training data at scale in the medical domain is often impractical~\cite{cohen2022torchxrayvision,bakator2018deep}, 
due to its safety-critical nature.
In this paper, we, therefore, explore an alternative by injecting medical expert knowledge into the visual representation learning procedure.

% To incorporate the prior knowledge, a na\"ive approach is to directly use the public text encoder that pre-trained on large medical corpus, 
% such as the electronic health records MIMIC III~\cite{Johnson2016MIMICIIIAF} or scientific publications PubMed, to guide the classification task.
% However, there exist several obstacles.
% First, the abstract and complex professional medical terminologies make it challenging for the text encoder to understand.
% Second, limited classes in common diagnosis datasets make the network easily overfit on the class-name embedding input, unable to indeed build the shared patterns across different classes based on prior knowledge.
% This is a fatal information loss for medical image analysis, 
% because, in manual diagnosis, beyond the images, the prior knowledge of the target pathology category also plays a vital role. 
% \weidi{this paragraph seems a bit redundant at the moment, 
% can directly say, we present a novel knowledge-enhanced .....}
% \weidi{actually, this paragraph can be a discussion in the experiment section, to explain why this naive approach is sub-optimal, e.g. Tab.2.}

%combining the language models into vision tasks provides a promising alternative in computer vision~\cite{zhou2022extract,thomason2014integrating}. 
%Especially for the classification tasks, introducing the class name embedding with pre-trained text encoder shows great potential to promote performance~\cite{radford2021learning,pratt2022does}.

% To incorporate the prior knowledge, a na\"ively approach is to directly use the public text encoder that pre-trained on large medical corpus, such as the electronic health records MIMIC III~\cite{Johnson2016MIMICIIIAF} or scientific publications PubMed, to guide the classification task.

% abstractness of many complex and professional medical terminologies makes high-quality textual representation learning more challenging.
% ignoring the information contained in the categories~\cite{cohen2022torchxrayvision,bakator2018deep}. 


% First, professional medical terminologies make it challenging to obtain a high-quality text encoder. 
% Second, limited classes in common diagnosis datasets make the network easily over-fit on the class-name embedding input, unable to indeed build the shared patterns across different classes.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/fig1_teaser.pdf}
    \vspace{-0.5cm}
    \caption{In the conventional training scheme~(left), 
    manual annotations are often converted into \textbf{discrete} one-hot vectors, 
    that are \textbf{orthogonal} in the embedding space, thus ignoring the implicit relations between labels. While in our proposed knowledge-enhanced classification framework (right), the labels are transformed into \textbf{continuous} vectors in a knowledge embedding space, to capture the implicit relations, and further used to supervise visual representation learning.
    %\weidi{this figure is abstract anyway, can we use the figure in the presentation, can polish it more, but that is clearer I think. }\xiaoman{update later}
    %\weidi{general comments, in the figure, make sure to emphasize the informative message. 
    %For example, readers in our community can easily get the image, visual encoder, so their size can be relatively small. }
    } 
    \label{fig:intuition}
    \vspace{-0.5cm}
\end{figure}

% \weidi{last two paragraphs are good.}
We present a novel knowledge-enhanced classification framework, as shown in the upper right of Fig.~\ref{fig:intuition}, {\em first}, to explicitly incorporate experts' knowledge,
we build a neural representation for the medical knowledge graph via contrastive learning, acting as a ``knowledge encoder'' that explicitly encodes the relations between medical concepts in the embedding space; 
%between positive and negative pairs generated from the knowledge base,
{\em second}, while training the visual encoder, we keep the parameters of the knowledge encoder frozen, and only learn a set of prompt vectors for efficient adaptation;
%inspired by the success of prompt learning, 
%we propose a knowledge-decompose module, regularizing the embedding space and forcing the network implicitly build the relationships between different classes based on the knowledge-enhanced text embedding.
%Specifically, we use a learnable to represent the shared hidden space across classes. For each pathology, the network can only use the linear combinations of the basis to represent it;
{\em third}, we adopt a Transformer-based disease-query module for text-image cross-modality fusion, where the disease names act as queries that cross-attend the visual features and infer the likelihood of the disease existence,
naturally, it enables explainable diagnosis results via the
cross attentions.
% \weidi{check this paragraph, see if it reads well.}
% \xiaoman{text-prompt, that can implicit decompose the textual contents and regularize the embedding space, -- benefits when combining different datasets/ new classes ?};

To demonstrate the effectiveness of the proposed knowledge-enhanced classification framework, we conduct thorough experiments to analyze from three perspectives:
{\em first}, we experiment on three disease diagnosis tasks across different anatomy structures, to show our method is efficient across various image distributions;
{\em second}, we train on a combination of 11 public chest x-ray datasets, 
showing our model can better exploit the potential of various public datasets regardless of their annotation granularity, 
which traditional training paradigm can slightly benefit from;
{\em third}, we perform zero-shot disease diagnosis, 
{\em i.e.}, evaluating unseen classes on PadChest~\cite{bustos2020padchest}, achieving an AUC of at least 0.600 on 79 out of 106 unseen radiographic findings, 
Note that, such a task is completely unachievable in conventional supervised training.

%\weidi{\textbf{general comments:} I noticed that you are using Transformer for disease classification, this is serving the topic, i.e., knowledge-enhanced learning, if you want to show we can also do grounding, this needs to be claimed in the introduction, and also need experiments to support it. } 
%\chaoyi{We will add a visualization for grounding to show we add this module to provide interpretability.}

==> miccai2023 (1)/contents/method.tex <==
\section{Method}
In this section, we start by describing the considered problem scenario in Sec.~\ref{sec:problem_scenario}, 
followed by the procedure of condensing the medical domain knowledge into a text encoder in Sec.~\ref{sec:text_encoder}.
In Sec.~\ref{sec:training}, we detail the proposed knowledge-enhanced classification model, including the visual encoder, knowledge encoder, 
learnable prompt module, and disease-query module, and describe the training procedure.
% text-prompting module
%
%\weidi{text-prompting is not good, think of another term}
%\xiaoman{knowledge-prompt module or attribute module? and the whole framework named as knowledge-enhanced classification framework?}



\subsection{Problem Scenario}
\label{sec:problem_scenario}
Given a dataset with $N$ sample pairs, 
{\em i.e.}, $\mathcal{D}_{\text{train}} = \{(x_1, y_1), (x_2, y_2),\dots, (x_N, y_N)\}$,
where ${x}_i \in \mathbb{R}^{H \times W \times 3}$ refers to the input image, 
and $y_i \in \mathcal{T}=\{t_1. \dots, t_Q \}$ denotes the ground truth annotation from a pool of $|Q|$ candidate diseases. Unlike conventional supervised learning that often converts the labels to one-hot vectors,
our goal is to train a classification model that leverages the semantics encapsulated in the disease category texts, specifically, 
\begin{align}
    {S}_i = \Phi_{\text{query}}(\Phi_{\text{visual}}({x}_i), \Phi_{\text{prompt}}(\Phi_{\text{knowledge}}(\mathcal{T}))),
\end{align}
where ${S}_i \in \mathbb{R}^{Q}$ refers to the inferred likelihood of the patient having any disease in $\mathcal{T}$.
$\Phi_{\text{knowledge}}(\cdot), \Phi_{\text{prompt}}(\cdot), \Phi_{\text{visual}}(\cdot),  \Phi_{\text{query}}(\cdot)$ refer to the trainable modules in our proposed knowledge-enhanced classification framework, that will be detailed in the following sections.
%\weidi{notation question, $\Phi_{\text{text}}$ or something related to knowledge encoder ?
%$\Phi_{\text{output}}$ or something related to the disease query module ?}
%\xiaoman{fixed}
%to the ground truth of all diseases in $\mathcal{T}=\{t_1. \dots, t_Q \}$, respectively.
% and the disease categories set $\mathcal{T}=\{t_1. \dots, t_Q \}$,
% ${x}_i \in \mathbb{R}^{H \times W \times 3}$ refers to an image with $H, W$ denoting height and width respectively,
% Let $\mathcal{T}=\{t_1. \dots, t_Q \}$ denotes the disease categories,
%\weidi{this scenario setup is confusing, there is no link between y and T.}
%\xiaoman{fixed}
% \textbf{Note that,.....}
% \xiaoman{when assembling diverse datasets, some classes are partially labeled, introduce how to address the partial label problem.}

% In this section, we introduce the proposed knowledge-enhanced text-prompt leaning method in detail.
% As shown in Fig.....
% given the disease categories $\mathcal{T}=\{t_1,t_2,...,t_Q\}$, 
% we first get the disease text embedding $\boldsymbol{T} = \{\boldsymbol{t}_1,\boldsymbol{t}_2,...,\boldsymbol{t}_Q\}$ with the medical knowledge-enhanced text encoder $\Phi_{\text{text}}$ , where $\boldsymbol{T} = \Phi_{\text{text}}(\mathcal{T})$.
% Then a text-prompt module $\Phi_{\text{prompt}}$ is designed to learn the shared pattern across different diseases, where $TP =\Phi_{\text{prompt}}(\boldsymbol{T})$.
% Moreover, a disease-query module $\Phi_{\text{query}}$ is proposed to identify the existence of the diseases:
% \begin{align}
%     {s}_i = \Phi_{\text{query}}(\Phi_{\text{image}}({x}_i), \Phi_{\text{prompt}}(\Phi_{\text{text}}(\mathcal{T}))),
% \end{align}
% where ${x}_i \in \mathbb{R}^{H \times W \times 3}$ refers to an image with $H, W$ denoting height and width respectively,
% ${s}_i \in [0, 1]$ refers to the inferred likelihood of the patient having a certain disease.
% In the following sections,
% we first introduce the training procedure of the medical knowledge enhanced text encoder.
% Then we detail the individual components of the proposed architecture,
% namely, the text encoder, text-prompt module, visual encoder, and disease-query module.


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{images/fig2_framework_1.pdf}
%     \caption{ The UMLS knowledge base used for training the text encoder~(left)workflow.
%     The framework of the Knowledge-enhanced text encoder~(right).
%     % \weidi{so we don't model relation any more? 
%     % I like the idea of inferring relationships between entities to encode knowledge.}
%     }
%     \label{fig:text_encoder}
%     \vspace{-0.3cm}
% \end{figure}

\subsection{Knowledge Encoder}
\label{sec:text_encoder}
To explicitly incorporate experts’ knowledge, 
we propose to inject the medical domain knowledge into a text encoder~($\Phi_{\text{knowledge}}$), by implicitly modeling the relations between medical entities in the textural embedding space.
Specifically, we employ an off-the-shelf knowledge graph in the medical community, 
namely, Unified Medical Language System~(UMLS)~\cite{bodenreider2004unified},
to fine-tune a pre-trained BERT language model. 
In the following section, we detail the training procedure, as shown in Fig.~\ref{fig:framework}.

\vspace{6pt} \noindent \textbf{Notation. }
Let $\mathcal{D}_{\text{UMLS}} = \{(n,d)_i\}_{i=1}^{||D||}$ denote a concept dictionary for UMLS in text form, 
each concept~($n_i$) is associated with one corresponding definition~($d_i$),
for example, the concept ``pulmonary infiltrate'' is defined as ``A finding indicating the presence of an inflammatory or neoplastic cellular infiltrate in the lung parenchyma''.

\vspace{6pt} \noindent \textbf{Training.~}
Here, we train the text encoder by maximizing the similarities between positive concept-definition pairs, 
{\em i.e.}, pull the distance of language description and its corresponding concept in the textual embedding space. Given $N$ randomly sampled concepts and definitions, 
we pass them through a standard BERT architecture~\cite{devlin2018bert},
and take the average-pooled features as their textual embeddings.
%\xiaoman{we can compute their textual embedding of corresponding language descriptions with average-pooling,}
{\em i.e.}, the concept~$\boldsymbol{n}_i \in \mathbb{R}^{N \times d}$, definition~$\boldsymbol{d}_i\in \mathbb{R}^{N \times d}$. 
% \weidi{average pooled ? or [CLS] token ?}
At training time,
each mini-batch can be expressed as $\{(n_i,d_i)\}_{i=1}^{N}$,
and the model can be trained via contrastive learning~\cite{oord2018representation}:
% \weidi{cite infoNCE}:
\begin{align}
\mathcal{L}_{\text{contrastive}} =  -\frac{1}{2N}\sum_{k=1}^{N}(\log \frac{e^{(\langle{\boldsymbol{n}}_i, {\boldsymbol{d}}_i\rangle/\tau)}}{\sum_{k=1}^{N} e^{(\langle{\boldsymbol{n}}_i, {\boldsymbol{d}}_k\rangle/\tau)}} + \log \frac{e^{(\langle{\boldsymbol{d}}_i, {\boldsymbol{n}}_i\rangle/\tau)}}{\sum_{k=1}^{N} e^{(\langle{\boldsymbol{d}}_i, {\boldsymbol{n}}_k\rangle/\tau)}}).
\end{align}
where $\tau \in \mathbbm{R}^{+}$ is a scalar temperature parameter.
Once this is trained, the text encoder effectively becomes a ``knowledge encoder'' with domain experts' knowledge injected.
%\weidi{give a short summary sentence, once this is trained, what are we gonna have.}
% pointed to the same 
%\weidi{I don't understand the above sentence, it sounds like, 
%there will be multiple language descriptions pointing to the same concept.}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{images/fig2_framework_3.pdf}
    \vspace{-0.6cm}
    \caption{Overview of the knowledge-enhanced disease diagnosis workflow. 
    The knowledge encoder~(left) is first trained to learn a neural representation of the medical knowledge graph via contrastive learning, 
    and then used to guide the visual representation learning in our knowledge-enhanced classification model~(right).
    %\weidi{a bit more details.}
    % \weidi{the size of the modules needs to be changed a bit,  for example, currently the text encoder, and visual encoder is quite large, without providing information, while the important parts are relatively small, for example, learnable prompt, knowledge, etc. }
    %\weidi{this figure is a bit too large, can we somehow combine figure 2 and 3 ?}
    %\xiaoman{combined}
    }
    \label{fig:framework}
    \vspace{-0.3cm}
\end{figure}

\subsection{Knowledge-enhanced Classification Model}
\label{sec:training}

%\weidi{\textbf{general comments:} why the math font is so ugly..... can we do better ?}
%\xiaoman{Update HF to h, P to p, TP change to k}
After injecting the domain knowledge into the text encoder, 
here, we describe the procedure to guide the visual representation learning with the knowledge encoder. 
Specifically, the classification model consists of four core modules, 
namely, the visual encoder, frozen knowledge encoder,
prompt module, and disease-query module.
%\weidi{same as previously mentioned, I don't like the name `text-prompt module'.}

\vspace{6pt} \noindent \textbf{Visual Encoder. }
Given an image scan $x_i \in \mathbb{R}^{H \times W \times 3}$,
we compute the features with a visual backbone, 
which can be either ResNet~\cite{he2016deep} or Vision Transformer~\cite{dosovitskiy2020vit},
$ \boldsymbol{x}_i = \Phi_{\text{visual}}({x}_i) \in \mathbbm{R}^{h\times w \times d}$,
%\begin{align}
%    \boldsymbol{x}_i = \Phi_{\text{image}}({x}_i) \in \mathbbm{R}^{m_x \times d},
%\label{xi}
%\end{align}
where $d$ refers to the feature dimension,
and $h, w$ denote the size of the output feature map,
feature dimension $d$ is set to 256.

%\weidi{why not simply write it as $\mathbbm{R}^{h \times w \times d}$ ?} \chaoyi{fixed}


\vspace{6pt} \noindent \textbf{Frozen Knowledge Encoder. }
Given the disease categories $\mathcal{T}$, 
we compute the features with the pre-trained knowledge encoder:
$\boldsymbol{T} = \Phi_{\text{knowledge}}(\mathcal{T}) \in \mathbbm{R}^{Q \times d}$,
%\begin{align}
%    \boldsymbol{T} = \Phi_{\text{text}}(\mathcal{T}) \in \mathbbm{R}^{Q \times d},
%\end{align}
where $d$ refers to the feature dimension, and $Q$ refers to the category number.
As the number of classes in downstream medical diagnosis datasets is usually extremely limited, \emph{e.g.}, 10 diseases on VinDr-Mammo~\cite{Nguyen2022VinDrMammoAL}, 
to prevent the knowledge encoder from over-fitting on certain training classes, 
deviating from the originally embedded knowledge graph,
we keep its parameters frozen, and use it to guide the learning of visual encoder, effectively, such a training procedure resembles knowledge injection into visual representation learning.

%Till here, we can directly use the disease embeddings to guide the learning of the visual encoder. However, 
%the model easily over-fitting on the training classes and cheating without indeed building the shared patterns. To further handle this, we propose to decompose the embedding spaces into a learnable basis, as detailed in the following.

%\weidi{we need to provide a link to the prompt,` till here, we can directly use the text embedding for ......, however, given the limited data, or what reason, to further ....., we propose to decompose the embedding spaces into learnable basis, as detailed in the following.' }


\vspace{6pt} \noindent \textbf{Learnable Prompt Module. }
To bring more flexibility, we also introduce a learnable prompt module~($\Phi_{\text{prompt}}$) for efficient knowledge adaptation.
%as described below. To further build the shared patterns across different diseases,
%we propose a knowledge-decompose module~($\Phi_{\text{prompt}}$). 
Specifically, as shown in the lower-right of Fig.~\ref{fig:framework},
it consists of a set of learnable vectors, {\em i.e.}, $\boldsymbol{h}\in \mathbbm{R}^{N \times d}$, where $N$ denotes the feature numbers and $d$ is the embedding dimension of each feature. 
%The parameters in $\boldsymbol{h}$ are all learnable during training. 
Given the disease embeddings~($\boldsymbol{T} \in \mathbbm{R}^{Q \times d}$), 
we first use an MLP to project it into a probability distribution over the learnable prompt vectors, $\boldsymbol{p} = \text{SoftMax}(\text{MLP}(\boldsymbol{T})) \in \mathbbm{R}^{Q \times N}$.
Then, the output of the Prompt Module can be calculated as the matrix multiplication between $\boldsymbol{p}$ and $\boldsymbol{h}$, 
{\em i.e.}, that can be formulated as 
$\boldsymbol{k} = \Phi_{\text{prompt}}(T) = (\boldsymbol{p} \cdot \boldsymbol{h}) \in  \mathbbm{R}^{Q \times d}$.

% To further build the shared patterns across different diseases, 
% we propose a text-prompt module~($\Phi_{\text{prompt}}$). It contains a hidden feature basis, 
% denote as $\boldsymbol{HF}\in \mathbbm{R}^{N \times d}$. $N$ denotes the feature numbers and $d$ is the embedding dimension of each feature. The parameters in $\boldsymbol{HF}$ are all learnable during training. Given the disease, text embedding $\boldsymbol{T} \in \mathbbm{R}^{Q \times d}$, we first use an MLP to project it into a probability distribution on the hidden feature basis, $\boldsymbol{P} = \text{SoftMax}(\text{MLP}(\boldsymbol{T})) \in \mathbbm{R}^{Q \times N}$.
% Then, the output of the Text-Prompt Module $\boldsymbol{TP} \in  \mathbbm{R}^{Q \times d}$ can be calculated as the mat-multiple of $\boldsymbol{P}$ and $\boldsymbol{HF}$,
% % $\boldsymbol{TP} = \langle \boldsymbol{P},\boldsymbol{HF} \rangle \in  \mathbbm{R}^{Q \times d}$, where $\langle \cdot,\cdot \rangle$ denotes the mat-multiple operation. 
% In general, the Text-Prompt Module can be formulated as $\boldsymbol{TP} = \Phi_{\text{prompt}}(T)$.


\vspace{6pt} \noindent \textbf{Disease-Query Module. }
We use a 4-layer transformer decoder with an MLP to get the final prediction. 
Given the disease categories $\mathcal{T}$,
we have converted them into a set of disease embeddings~($\boldsymbol{k}$) with the pre-trained knowledge encoder and learnable prompt module.
As inputs to the Transformer decoders,
disease embeddings are treated as \texttt{queries},
and the encoded features~($\boldsymbol{x}_i$) act as \texttt{key} and \texttt{value} of the disease-query module:
${s}_i = \Phi_{\text{query}}(\boldsymbol{x}_i, \boldsymbol{k}) \in \mathbbm{R}^{Q \times C}$, 
where $C$ represents the class number and is set as 2, 
since the diagnosis tasks are all binary classification.
% \weidi{well, this verifies my early assumption, but why not write it in the method section ?} 
Cross-entropy loss is used as the optimization function.
%\weidi{I don't understand the output here, why it is by C dimension ? I thought it's binary ? indicating the likelihood of certain disease ?}

%outputs a response for each query, {\em i.e.} identifying the disease.
%\begin{equation}
%\end{equation}
%\weidi{check the general comments, need to specify the motivation of using this, and experiments to validate its usefulness.}
%\xiaoman{add grounding visualization later.}

==> miccai2023 (1)/contents/results.tex <==
\section{Results}
% The goal of the proposed method is to leverage medical expert knowledge to improve the disease diagnosis task.
Here, we conduct experiments to validate the effectiveness of our knowledge-enhanced classification model.
In Sec.~\ref{sec:result1}, we first compare knowledge-enhanced training with standard training using discrete labels across different architectures and then perform a thorough ablation study of proposed modules.
In Sec.~\ref{sec:result2}, we conduct an analysis on the proposed knowledge encoder by replacing it with other pre-trained language models. In Sec.~\ref{sec:result3}, we experiment on \textbf{CXR-Mix}, 
to show that our model can effectively exploit knowledge across datasets with varying annotation granularity, we conduct analysis from three aspects: 
(i) the ability to combine various partial-labeled datasets, 
(ii) to leverage implicit relations between diseases, 
(iii) to diagnose diseases that are unseen at training time, 
resembling an open-set recognition scenario.  
%\weidi{The results are not structured at the moment, difficult for readers to keep track.}

%\weidi{first write down the logics here, 
%(1) knowledge-enhanced training vs.~standard training with discrete labels, architecture comparison.
%(2) knowledge encoder, pre-trained llm vs.~ours with knowledge graph injected.
%(3) analysis on CXR-Mix, to show our model can effectively exploit knowledge across datasets, annotation granularity.
%(4) class diversity, isn't this a special case of (3) ? 
%(5) zero-shot, again, to me, this is a special case of (3).
%(6) no discussions for grounding visualisation.}
%\xiaoman{the grounding visualisation is included in the ablation study section.}

% and the knowledge-enhanced text-encoder in Sec.~\ref{sec:result2} on three diagnosis datasets across different anatomy structures.
% Then in Sec.~\ref{sec:result3} we show the superior performance of the proposed method when we assemble different public chest X-ray datasets, in Sec.~\ref{sec:result4} analyze the benefits from two perspectives: ``Diversity'' and ``Amount'' and \chaoyi{in Sec.~\ref{result5} further analyse the ability to handle open-set unseen diseases.}
%\weidi{TO CONTINUE .....}




\vspace{-0.2cm}
\subsection{Analysis of Knowledge-Enhanced Classification Model}
\label{sec:result1}

% In this section, we compare the proposed knowledge-enhanced classification model with baseline classification models and conduct an ablation experiment to evaluate the effectiveness of each component, including the text encoder~(TE) and knowledge-decompose module~(DM).
\subsubsection{Comparison to Conventional Training Scheme.}
As baselines, we adopt the widely used ResNet-50~\cite{he2016deep} and ViT-16~\cite{dosovitskiy2020image},
and train with conventional learning scheme, {\em i.e.}, using discrete labels.
The results are summarized in Tab.~\ref{resnet}, 
we refer the reader to detailed results for each category presented in the supplementary material~(Tab.~\ref{pcxr},~\ref{spinexr} and ~\ref{mammo}). 
Our proposed knowledge-enhanced model achieves a higher average AUC on all three datasets across different architectures.


\begin{table}[t]
\caption{Compare with Baseline Models with ResNet-50~\cite{he2016deep} and ViT-16~\cite{dosovitskiy2020vit}  as backbone on disease classification tasks.
KE indicates the proposed knowledge encoder, LP indicates the proposed learnable prompt module, and the number denotes the prompt number.
AUC scores averaged across different diseases are reported. We report the mean and standard deviation of three different seeds.}
\vspace{-5pt}
%\weidi{unify the terminologies according to method section, for example TE --> knowledge encoder, DM --> learnable prompt}
\centering
\setlength{\tabcolsep}{5pt}
\footnotesize
\begin{tabular}{llcc|ccc}
\toprule
Model & Backbone & KE & LP & VinDr-PCXR & VinDr-Mammo & VinDr-SpineXr  \\
\midrule
Res~\cite{he2016deep} & ResNet-50 & \xmark  & \xmark & 70.53 $\pm$ 1.00 &  82.54 $\pm$ 1.79  & 87.35 $\pm$ 0.38 \\
Res+KE & ResNet-50 & \cmark  &  \xmark & 71.39 $\pm$ 0.66 & 83.23 $\pm$ 1.98 & 87.76 $\pm$ 0.41  \\
Res+KE+LP & ResNet-50 & \cmark & 32 & \textbf{73.97 $\pm$ 0.28} &  80.59 $\pm$ 3.11 & 88.46 $\pm$ 0.22 \\
Res+KE+LP & ResNet-50  & \cmark  & 64 & 72.88 $\pm$ 0.19 &  81.27$\pm$ 1.83  & \textbf{88.90 $\pm$ 0.04 } \\
Res+KE+LP & ResNet-50 & \cmark  & 128 & 73.70 $\pm$ 0.41 & \textbf{ 84.80 $\pm$ 1.04 } & 88.22 $\pm$ 0.53  \\
\midrule
ViT~\cite{dosovitskiy2020vit} & ViT-16 & \xmark   & \xmark & 69.06$\pm$ 0.74 & 80.50 $\pm$ 2.47 & 85.56 $\pm$ 0.97  \\
ViT+KE & ViT-16 & \cmark   & \xmark  & 71.69 $\pm$ 1.64 & 83.89 $\pm$ 0.38  & 85.75 $\pm$ 0.44  \\
ViT+KE+LP & ViT-16 & \cmark  & 32 & \textbf{72.90 $\pm$ 0.97} & 83.67 $\pm$ 2.34 & 86.55 $\pm$ 0.48 \\
ViT+KE+LP & ViT-16 & \cmark  & 64 &  71.07 $\pm$ 3.28 & 84.33 $\pm$ 1.54 & \textbf{86.83 $\pm$ 0.81} \\
ViT+KE+LP & ViT-16 & \cmark  & 128 & 72.47 $\pm$ 0.78 & \textbf{84.46 $\pm$ 0.84 }& 86.33 $\pm$ 0.23  \\
\bottomrule
\end{tabular}
\label{resnet}
\vspace{-0.4cm}
\end{table}

\vspace{-0.3cm}
\subsubsection{Ablation Study.}
We conduct a thorough ablation study of the proposed model by removing individual modules and varying the hyper-parameters, as shown in Tab.~\ref{resnet}.
Specifically, the performance of ResNet-50 is improved to $71.39\%$, $83.23\%$, and $87.76\%$ for the three different tasks equipped with the proposed knowledge encoder to guide the visual representation learning.
While combining with the learnable prompt~(LP) module, which potentially offers more flexibility for knowledge adaptation, we observe a significant performance gain, up to $2.58\%$ on average AUC scores on VinDr-PCXR.
The same conclusion can be drawn for the ViT-16 visual backbone.

To analyze the effect of prompts, we experiment with different numbers of prompts.
As shown, the optimal number of prompts varies from task to task, but in general, adding the LP module benefits all the downstream tasks.
The only exception is for the VinDR-Mammo task with ResNet as a backbone,
which is mainly caused by the extremely small test samples in some categories~(Tab.~\ref{mammo}), {\em e.g.}, skin retraction and skin thickening.
%\weidi{need a sentence on the number of prompts, especially on VinDR-Mammo, why it is sometimes lower with prompts. }
% In general, adding the LP module benefits downstream tasks, except that

\vspace{-0.3cm}
\subsubsection{Qualitative Visualisation.}
To provide a visualization that can potentially be used for clinicians to discover and understand the evidence that AI algorithm bases its predictions on,
the disease-query module in our proposed architecture enables detailed visualization for each of the queries with positive output.
Specifically, we average the cross-attention map in each transformer layer in the disease query module, and visualize the results in Fig.~\ref{fig:visualize}.
The model's attention well matches radiologists’ diagnoses of different diseases, 
{\em i.e.} red boxes labeled by board-certified radiologists.


\begin{figure}[!htb]
    \centering
    \includegraphics[width=.97\linewidth]{images/visualize.png}
    \vspace{-0.4cm}
    \caption{Sample visualization of randomly chosen samples from VinDr-SpinXr, 
    we present both the original image (left) and an attention map generated from our proposed model with ResNet-50 as the backbone (right). }
    \label{fig:visualize}
    \vspace{-0.3cm}
\end{figure}


% In this section, we compare the proposed knowledge-enhanced classification model with baseline classification models and conduct an ablation experiment to evaluate the effectiveness of each component, including the text encoder~(TE) and knowledge-decompose module~(DM).
% As baselines we consider the widely used ResNet-50~\cite{he2016deep} and ViT-16~\cite{dosovitskiy2020image}.
% \textcolor{blue}{``TE'' refers to the use the proposed knowledge-enhanced text encoder for classification without using the text prompt module, and  ``KD'' represents the whole knowledge-enhanced classification model.}
% \weidi{not clear to me if text encoder our knowledge-enhanced one or simply encoding class names with pre-trained BERT, as the title in this section is something called `text-enhanced', the terminology is confusing.}
% The results are summarized in Tab.~\ref{resnet}.
% The detail results of each category are presented in the supplementary material.
% As shown, the performance is improved to $71.39\%$, $83.23\%$, $87.76\%$, $83.33\%$ for the four different tasks equipped with the proposed knowledge text encoder on the ResNet-50.
% While combined with the knowledge-decompose module, 
% the model implicitly learns to decompose and re-link the disease categories in the textual embedding space.
% A significant performance gains up to $2.58\%$ in average AUC scores on VinDr-PCXR confirms the effectiveness of the knowledge-decompose module. 
% We can draw the same conclusion that the adoption of the two modules yields much better results than simply classification from the results with ViT-16 as backbone.


\subsection{Analysis of the Knowledge-Enhanced Text Encoder}
\label{sec:result2}
Here we investigate another way of incorporating prior knowledge,
that is, to guide the visual representation with a text encoder pre-trained on the large medical corpus,
%To incorporate the prior knowledge, a na\"ive approach is to directly use the public text encoder that is pre-trained on the large medical corpus, 
such as the electronic health records MIMIC III~\cite{Johnson2016MIMICIIIAF} or scientific publications PubMed, to guide the classification task.
As shown in Tab.~\ref{ablation},
while comparing with the models that adopts ClinicalBERT~\cite{alsentzer2019publicly} or PubMedBERT~\cite{gu2021domain} as knowledge encoder, we can make two observations:
(i) guiding visual representation learning with domain knowledge generally works better,
{\em e.g.}, results of using ClinicalBERT or PubMedBERT outperform conventional training with discrete labels, 
(ii) our proposed knowledge-enhanced text encoder consistently demonstrates superior results, that can be attributed to the explicitly injected domain knowledge, rather than implicitly learning it from the document corpus.
% \weidi{check the above paragraph.}x

%When we use other text encoder, like ClinicalBERT, only a small gain of $0.30\%$ on AUC compared with simple classification on VinDr-PCXR.
%And the similar situation occurs on other target tasks.
%Unsurprisingly, the highest overall results are obtained by applying the proposed knowledge-enhanced text encoder, proving the effectiveness of introducing expert knowledge in the text encoder.
%However, there exist several obstacles as the abstract and complex professional medical terminologies make it challenging for the text encoder to understand.

\vspace{-0.2cm}
\begin{table}[!htb]
\caption{Ablation study on knowledge encoder with ResNet as a backbone, 
mean and standard deviation for AUC scores is reported with three different seeds.
we use the optimal prompt numbers according to the ablation study, 
{\em i.e.}, 32 for VinDr-PCXR, 128 for VinDr-Mammo, and 64 for VinDr-SpineXr.}
\vspace{-0.2cm}
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lc|ccc}
\toprule
Model & Knowledge Encoder  & VinDr-PCXR & VinDr-Mammo & VinDr-SpineXr \\
\midrule
Res~\cite{he2016deep} & - & 70.53 $\pm$ 1.00 &  82.54 $\pm$ 1.79  & 87.35 $\pm$ 0.38 \\
Res+KE+LP & ClinicalBERT~\cite{alsentzer2019publicly}  & 70.83 $\pm$ 0.96 & 83.55 $\pm$ 0.72 & 88.19 $\pm$ 0.25\\
Res+KE+LP & PubMedBERT~\cite{gu2021domain}& 71.73 $\pm$ 0.75  & 81.96 $\pm$ 1.82 & 88.25 $\pm$ 0.65 \\
Res+KE+LP & Ours & \textbf{73.97 $\pm$ 0.28} & \textbf{84.80 $\pm$ 1.04} & \textbf{88.90 $\pm$ 0.04 }\\
% ResNet-stanfordgpt & 72.06 $\pm$ 0.73 & 80.24 $\pm$ 2.48 & 87.55 $\pm$ 0.27 & 79.95 $\pm$ 1.16 \\
\bottomrule
\end{tabular}
\label{ablation}
\vspace{-0.4cm}
\end{table}


\subsection{Analysis on the CXR-Mix}
\label{sec:result3}

In this section, we experiment on the assembled dataset \textbf{CXR-Mix}, 
to demonstrate the effectiveness of our proposed framework in exploiting knowledge across datasets and annotation granularity. 

\subsubsection{The Ability to Combine Various Partial-labeled Datasets: }
Unlike the traditional approach, which requires to carefully merging the label space from different datasets~\cite{cohen2022torchxrayvision,cohen2020limits,lambert2020mseg} to benefit from them, 
our formulation of embedding the `disease name' with a knowledge encoder naturally enables us to train models on the mixture of multiple datasets, handling different granularities of diagnosis targets and inconsistent pathology expression. 
As shown in Tab.~\ref{Assembling results}, we compare to TorchXRayVision~\cite{cohen2022torchxrayvision} that merges the label space 
and trains a baseline model with discrete labels, 
our knowledge-enhanced framework improves the performance from $82.60\%$ to $85.13\%$ and form $77.39\%$ to $79.54\%$ under the two commonly-used backbones, ResNet and ViT, respectively. 
%The gain of each module is also presented in Tab.~\ref{Assembling results}. The results demonstrate our framework is more suitable for assembling datasets. 

\vspace{-0.4cm}
\begin{table}[!htb]
\centering
\caption{Compare with Baseline Models on disease classification tasks on the assembling dataset. AvgAUC refers to the AUC score averaged across different diseases. The first line refers to the use of the training flow proposed by TorchXrayVision~\cite{cohen2022torchxrayvision} and use ResNet or ViT as the backbone.}
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lcc|lcc}
\toprule
Methods & Prompt &AvgAUC  & Methods & Prompt & AvgAUC \\ \toprule

Res~\cite{cohen2022torchxrayvision}      & -        & 82.60 $\pm$ 1.27  & ViT~\cite{cohen2022torchxrayvision} & - & 77.39 $\pm$ 0.71\\
%ResNet\_xmbert              & 0.8333  & ViT\_xmbert & -\\
%ResNet\_GPT              & 0.8284  & ViT\_GPT & -\\
Res+KE      & -   & 83.11 $\pm$ 0.27   & ViT+KE & - & 78.30 $\pm$ 0.93\\
Res+KE+LP     & 32   &   84.45 $\pm$ 1.06 & ViT+KE+LP  & 32 & 79.25 $\pm$ 1.05\\
%ResNet\_xmbert \&Image\_prompt\_DQN & 0.8316   & ViT\_xmbert \&Image\_prompt\_DQN & -\\
Res+KE+LP     & 64   & \textbf{85.13} $\pm$  0.78 & ViT+KE+LP   & 64& \textbf{79.54 $\pm$ 0.60}\\
Res+KE+LP       & 128   & 83.38 $\pm$  0.18& ViT+KE+LP  & 128 & 78.42 $\pm$ 0.71\\ \bottomrule
\end{tabular}
\label{Assembling results}
\vspace{-1.0cm}
\end{table}

\subsubsection{The Ability to Leverage Class Diversity: }
In this part, we further show that our framework can significantly improve the performance of each dataset, by training on data from other categories. 
Specifically, we consider each dataset separately, \emph{i.e.}, measuring the performance on their own test splits. We propose to decouple the data increment into two dimensions, ``Diversity'' and ``Amount''. ``Diversity'' refers to only adding the cases beyond the target classes and keeping the amount of data of target classes constant, while  ``Amount'' refers to increasing the target class cases. As shown in Fig.~\ref{fig:Results across P}, based on our structure, adding ``Diversity'' can improve the results on all 11 datasets. 
In particular, for some relatively small datasets, the gain is more significant, \emph{e.g.}, GoogleNIH, SIIM-ACR, and OpenI. 
Such an experiment has validated that a knowledge-enhanced model enables to leverage of the shared information between classes, and can be greatly beneficial for dealing with long-tailed diseases, which are seldom annotated in common datasets, 
by leveraging the publicly available data.

%Intuitively, such an experiment has validated our assumption that the knowledge-enhanced model enables to leverage the shared information between classes.



\vspace{-0.3cm}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/barplot.png}
    \vspace{-0.9cm}
    \caption{Analyse the performance gain on the assembling dataset.  
    % ``ResNet\_bar'' means the best performance ResNet baseline can achieve by leveraging the entire assembling dataset.
    ``Seperation'' refers to using a single dataset to train our framework. ``+Diversity'' refers to adding the cases beyond the target classes, increasing the class diversity, and keeping the data amount of the target classes constant. ``+Diversity+Amount'' means directly mixing the 11 datasets and for most datasets, the data amount of the target classes will further increase.
    }
    \label{fig:Results across P}
    \vspace{-0.6cm}
\end{figure}



\subsubsection{The Ability to Diagnose Open-set Unseen Diseases: }
Conventional models can only handle a close-set classification, while, with knowledge-enhanced design, our model enables to predict open-set diseases that never appear in the training set. 
This is meaningful for clinical practical usage, 
as some rare or new diseases can hardly find an off-shelf dataset to re-train models. We test our model on the PadChest testset~\cite{bustos2020padchest} 
and dismiss the classes that exist in the assembling dataset and those having very few cases~($n<=50$), that can hardly have statistically convincing test results. 
During testing, to get the embedding, we simply input the names of unseen classes into the knowledge encoder, and continue the standard evaluation procedure, {\em i.e.}, learnable prompt module, disease-query module. As shown in Fig.~\ref{fig:padchest}, without any example in the training set,  our model can directly achieve an AUC of at least $0.800$ on $14$ findings, at least $0.700$ on $46$ findings and at least $0.600$ on $79$ findings~(unseen at training time) out of 106 radiographic findings. 
This demonstrates our model can break the limits of the labeling classes and be adapted to more practical medical scenarios.


\vspace{-0.5cm}
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{images/padchest.pdf}
    \vspace{-.8cm}
    \caption{AUC and $95\%$ CI are shown on the unseen classes under the zero-shot setting. $n$ represents the number of related cases. The top 46 classes are plotted in the figure to show what classes our model can achieve $\text{AUC}>0.700$ on. Generally, our method achieves an AUC of at least 0.800 on 14 findings and at least 0.600 on 79 findings out of 106 radiographic findings where $n>50$ in the PadChest test dataset ($n=39,053$).}
    \label{fig:padchest}
    \vspace{-0.6cm}
\end{figure}

